QSym$^2$: A Quantum Symbolic Symmetry Analysis Program for Electronic Structure

Symmetry provides a powerful machinery to classify, interpret, and understand quantum-mechanical theories and results. However, most contemporary quantum chemistry packages lack the ability to handle degeneracy and symmetry breaking effects, especially in non-Abelian groups, nor are they able to characterize symmetry in the presence of external magnetic or electric fields. In this article, a program written in Rust entitled QSym$^2$ that makes use of group and representation theories to provide symmetry analysis for a wide range of quantum-chemical calculations is introduced. With its ability to generate character tables symbolically on-the-fly, and by making use of a generic symmetry-orbit-based representation analysis method formulated in this work, QSym$^2$ is able to address all of these shortcomings. To illustrate these capabilities of QSym$^2$, four sets of case studies are examined in detail in this article: (i) high-symmetry $\textrm{C}_{84}\textrm{H}_{64}$, $\textrm{C}_{60}$, and $\textrm{B}_9^-$ to demonstrate the analysis of degenerate molecular orbitals (MOs); (ii) octahedral $\textrm{Fe(CN)}_6^{3-}$ to demonstrate the analysis of symmetry-broken determinants and MOs; (iii) linear hydrogen fluoride in a magnetic field to demonstrate the analysis of magnetic symmetry; and (iv) equilateral $\textrm{H}_3^+$ to demonstrate the analysis of density symmetries.

==> suppinfo/preamble.tex <==
% ========
% Preamble
% ========



% ------------------
% Scientific support
% ------------------
% Chemistry
\usepackage[version=4]{mhchem}

% Scientific typesetting
\usepackage{siunitx}
\DeclareSIUnit{\atomicunit}{a.u.}
\DeclareSIUnit\atomicmassunit{u}
\DeclareSIUnit\angstrom{\text {Å}}

% -------------
% Maths support
% -------------
\usepackage{%
  amsthm,%
  amssymb,%
  mathrsfs,%
  mathtools,%
  gensymb,%
  braket,%
  mleftright,%
  nicefrac,%
  interval%
}
\intervalconfig{%
  soft open fences%
}

\mleftright

\newcommand*\bmmax{2}
\usepackage{bm}


% --------
% Diagrams
% --------

% Colours
\usepackage[usenames, svgnames, x11names, rgb]{xcolor}

% Graphics
\usepackage{graphicx}
\usepackage{grffile}

% TikZ & PGFPlots
\usepackage{pgfplots}

% Set up tikzexternalize
\usetikzlibrary{external}
\tikzexternalize
% \tikzexcmd is defined in the compilation call from the command line. See the Makefile.
\newif\iftikzex
\ifdefined\notikzex
  \tikzexfalse
\else
  \tikzextrue
\fi

\iftikzex
  \pgfplotsset{compat=1.18}

  \usetikzlibrary{
    calc,
    luamath,
    positioning,
    decorations.pathreplacing,
    backgrounds,
    arrows.meta,
    pgfplots.groupplots,
    pgfplots.patchplots,
    3d,
  }

  \usepgfplotslibrary[colormaps]

  \pgfplotscreateplotcyclelist{coloronly}{
    {red},
    {blue},
    {black!60!green},
    {black!20!orange},
    {black!30!blue},
    {green!30!brown},
    {blue!40!red},
    {IndianRed},
    {black!40!yellow},
    {Magenta4},
    {DodgerBlue4},
    {Maroon4},
    {Firebrick4},
    {Cyan4},
  }
\fi
\tikzexfalse

% Plot conditionals
\usepackage{xifthen}


% --------
% Captions
% --------
\usepackage{caption, subcaption}


% ------
% Tables
% ------
\usepackage{%
  booktabs,%
  array,%
  adjustbox,%
  makecell,%
  multirow,%
  bigdelim%
}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}m{#1}}

% -----
% Items
% -----
\usepackage[inline]{enumitem}


% --------
% Theorems
% --------
\theoremstyle{plain}
\newtheorem{proposition}{Proposition}
\theoremstyle{remark}
\newtheorem*{remark}{Remark}


% ----------
% Hyperlinks
% ----------
\usepackage[%
  hyperfootnotes=false,%
  hypertexnames=false,%
  hidelinks,%
]{hyperref}
\hypersetup{%
  bookmarksnumbered=true,%
  colorlinks=true,%
  citecolor=teal,%
  linkcolor=Blue4,%
}


% ------------
% Bibliography
% ------------
\usepackage{mciteplus}

% ---------
% Debugging
% ---------
%\listfiles
